Classifying fusion categories $\otimes$-generated by an object of small Frobenius-Perron dimension

The goal of this paper is to classify fusion categories $\otimes$-generated by a $K$-normal object (defined in this paper) of Frobenius-Perron dimension less than 2. This classification has recently become accessible due to a result of Morrison and Snyder, showing that any such category must be a cyclic extension of a category of adjoint $ADE$ type. Our main tools in this classification are the results of Etingof, Ostrik, and Nikshych, classifying cyclic extensions of a given category in terms of data computed from the Brauer-Picard group, and Drinfeld centre of that category, and the results of the author, which compute the Brauer-Picard group and Drinfeld centres of the categories of adjoint $ADE$ type. Our classification includes the expected categories, constructed from cyclic groups and the categories of $ADE$ type. More interestingly we have categories in our classification that are non-trivial de-equivariantizations of these expected categories. Most interesting of all, our classification includes three infinite families constructed from the exceptional quantum subgroups $\mathcal{E}_4$ of $\mathcal{C}( \mathfrak{sl}_4, 4)$, and $\mathcal{E}_{16,6}$ of $\mathcal{C}( \mathfrak{sl}_2, 16)\boxtimes \mathcal{C}( \mathfrak{sl}_3,6)$.

==> arXiv Final/preamble.tex <==
%!TEX root=Normal.tex
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.

\usepackage{amssymb, manfnt}
\usepackage{hyperref}
\usepackage[normalem]{ulem}
\usepackage{tikz}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{MnSymbol}
\usepackage{graphicx}
\usepackage{tikz-cd}
\usepackage{longtable}
\usepackage{amsmath,amscd,amsthm}
\usepackage{tkz-graph}
\tikzstyle{vertex}=[circle, draw, inner sep=0pt, minimum size=6pt]
\newcommand{\vertex}{\node[vertex]}
\usepackage[all]{xy}
\graphicspath{ {graphs/} }
\usetikzlibrary{decorations.text}
\usepackage{graphicx}
\usepackage[outdir=./pictures]{epstopdf}
\graphicspath{ {pictures/} }
\usepackage[all]{xy}
\usepackage{adjustbox}
%\usepackage{lmodern}
\usepackage{graphicx}
\usepackage{fullpage}
\usepackage[T1]{fontenc}
%\usepackage{microtype}
\usepackage{ifthen}
%\usepackage{libertine}
%\usepackage[libertine]{newtxmath}
\usepackage[all]{xy}
\usepackage{pdflscape}
\usepackage{array}
\usepackage{multirow}
\usepackage{rotating}


\def\altdb{\vadjust{\vbox to 0pt{\vss\hbox{\kern \hsize
\quad{\dbend}}\kern\baselineskip\kern-10pt}}}

\setlength{\textheight}{23cm} \setlength{\topmargin}{0cm}
\setlength{\textwidth}{16cm} \setlength{\oddsidemargin}{0cm}
\setlength{\evensidemargin}{0cm}


%\font\fiverm=cmr5
%Want to be able to change fields from blackboard bold to math bold easily. Hence the \field command
\newcommand\field[1]{\mathbb{#1}}
%Define all field macros
\newcommand\CC{\field{C}}
\newcommand\NN{\field{N}}
\newcommand\QQ{\field{Q}}
\newcommand\TT{\field{T}}
\newcommand\ZZ{\field{Z}}
%Define math calligraphic macros

\newcommand{\arxiv}[1]{\href{http://arxiv.org/abs/#1}{\tt arXiv:\nolinkurl{#1}}}
\newcommand{\doi}[1]{\href{http://dx.doi.org/#1}{{\tt DOI:#1}}}
\newcommand{\euclid}[1]{\href{http://projecteuclid.org/getRecord?id=#1}{{\tt #1}}}
\newcommand{\mathscinet}[1]{\href{http://www.ams.org/mathscinet-getitem?mr=#1}{\tt #1}}
\newcommand{\googlebooks}[1]{(preview at \href{http://books.google.com/books?id=#1}{google books})}
\newcommand{\zentralblatt}[1]{\href{http://www.zentralblatt-math.org/zmath/en/advanced/?q=#1&format=complete}{\tt #1}}
\newcommand{\numdam}[1]{\href{http://www.numdam.org/numdam-bin/item?id=#1}{\tt Numdam: #1}}



\makeatletter
\let\@@pmod\pmod
\DeclareRobustCommand{\pmod}{\@ifstar\@pmods\@@pmod}
\def\@pmods#1{\mkern4mu({\operator@font mod}\mkern 6mu#1)}
\makeatother
 
% \newcommand\subcat[1]{\operatorname{Diag}({#1})}
  \newcommand\subcat[1]{\underline{#1}}
  
\newcommand\dimHom{\operatorname{dimHom} }
\newcommand\Vect{\operatorname{Vect }}
\renewcommand\ker{\operatorname{ker}}
\newcommand\FPdim{\operatorname{FPdim}}
%\newcommand\Aut{\operatorname{Aut}}
\newcommand\Out{\operatorname{Out}}
\renewcommand\Vec{\operatorname{Vec }}
\newcommand\IVec{\operatorname{Vec }^{-}}
\newcommand\LVec{\operatorname{Vec }}
\newcommand\sVec{\operatorname{sVec }}
\newcommand\Fun{\operatorname{Fun}}
\newcommand\BrPic{\operatorname{BrPic}}
\newcommand\Obj{\operatorname{Obj}}
\newcommand\dims{\operatorname{dim}}
\newcommand\Mor{\operatorname{Mor}}
\newcommand\id{\operatorname{id}}
\newcommand\Aut{\operatorname{Aut}}
\newcommand\TenAut{\operatorname{Eq}}
\newcommand\Rep{\operatorname{Rep}}
\newcommand\Ind{\operatorname{Ind}}
\newcommand\Id{\operatorname{Id}}
\newcommand\Hom{\operatorname{Hom}}
\newcommand\range{\operatorname{range}}
\newcommand\ad{\operatorname{Ad}}
\newcommand\BrAut{\operatorname{EqBr}}
\newcommand\bal[1]{{#1} *_d {#1}}
\newcommand{\cs}{\ensuremath{C^{*}}}
\newcommand\Z[1]{ \mathbb{Z}_{#1}}

\newcommand\lie[1]{ \mathfrak{#1}}
\newcommand\cC{ \mathcal{C}}
\newcommand\cM{ \mathcal{M}}
\newcommand\cZ{ \mathcal{Z}}
\newcommand\cF{ \mathcal{F}}
\newcommand\cat[3]{ \cC(   \mathfrak{#1}_{#2} , #3)    }




\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem*{prop*}{Proposition}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{conj}[theorem]{Conjecture}
\newtheorem{rmk}[theorem]{Remark}
\theoremstyle{remark}



\newtheorem{rmks}[theorem]{Remarks}
\newtheorem{note}[theorem]{Note to selves}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\theoremstyle{definition}
\newtheorem{dfn}[theorem]{Definition}
\newtheorem{cons}[theorem]{Construction}
\newtheorem{dfns}[theorem]{Definitions}
\newtheorem{notation}[theorem]{Notation}
\newcommand\Inv{\operatorname{Inv}}
\newcommand{\nn}[1]{{\color{red}[[#1]]}}

\newcommand{\mm}[1]{{\color{red}{#1}}}

\newcommand{\highlight}[1]{{\color{red}#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{color}
\def\loc{\textcolor{blue}}
\def\aschange{\textcolor[RGB]{180,0,180}}
\def\mtchange{\textcolor[RGB]{20,160,50}}
\def\cfchange{\textcolor[RGB]{160,20,50}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\numberwithin{equation}{section}



\DeclareRobustCommand*{\nicefrac}{\@UnitsNiceFrac}%
\makeatother

